Generic Multilayer Network Data Analysis with the Fusion of Content and Structure

Multi-feature data analysis (e.g., on Facebook, LinkedIn) is challenging especially if one wants to do it efficiently and retain the flexibility by choosing features of interest for analysis. Features (e.g., age, gender, relationship, political view etc.) can be explicitly given from datasets, but also can be derived from content (e.g., political view based on Facebook posts). Analysis from multiple perspectives is needed to understand the datasets (or subsets of it) and to infer meaningful knowledge. For example, the influence of age, location, and marital status on political views may need to be inferred separately (or in combination). In this paper, we adapt multilayer network (MLN) analysis, a nontraditional approach, to model the Facebook datasets, integrate content analysis, and conduct analysis, which is driven by a list of desired application based queries. Our experimental analysis shows the flexibility and efficiency of the proposed approach when modeling and analyzing datasets with multiple features.

==> ses6_efficiency.tex <==
%Old: Multilayer networks have allowed for flexible composition of layers, as shown in the previous section, to support the analysis of the Facebook dataset from multiple perspectives. In order to perform each analysis for a query, communities had to be generated corresponding to various AND-compositions. In the remainder of the section, we will discuss how using EFF-COMM (node intersection based community generation method) of re-using the layer-wise communities is computationally better than the NA\"{I}VE-COMM approach that needs to generate graphs for each AND-composition for finding communities, by providing complexity analysis of the two approaches (Section \ref{subsec:complexity}) and experimental results (Section \ref{subsec:experiments}.)
This section discusses how the adapted approach, \textit{EFF-COMM}, of re-using the layer-wise communities is computationally better than the \textit{NA\"{I}VE-COMM} approach. In brief, \textit{NA\"{I}VE-COMM} is less efficient since for every analytical query listed in Section \ref{sec:problem-statement}, it has to generate graphs for each \textit{AND}-composition to find communities. %We provide complexity analysis of the two approaches (Section \ref{subsec:complexity}) and experimental results (Section \ref{subsec:experiments}.)

%sharma: even if you want to keep the analysis, i feels the algrorithms and the perf graph are redundant. Even the analysis is somewhat superficial and not complete! we have to express it as AND of M choose k if we want to be accurate. I think either we should refine 7.1 to make it complete and accurate or just keep 7.2. Then we can keep fig 9 as well.

%%you cannot put complexity in terms of computations whose complexity is not articulated! so i suggest we keep only sec 7.2. it will also come under slightly under 8 pages.

\subsection{Complexity Analysis}
\label{subsec:complexity}

For the complexity analysis, we assume that for a given multilayer network with fixed number of $M$ layers, say $\{G_1, \cdots, G_M\}$, each of the $N$ analytical queries  requiring ${K}$ related layers on average, should return a list of communities, $L$ (see Alg. 1).%~\ref{alg:naive_and_effective_approach}.

\begin{comment}

\end{comment}
\begin{figure}[!t]
\vspace{-20pt}
\scalebox{0.84}{
	\begin{minipage}[t]{14cm}%6cm <==========================================
		\vspace{2pt}
		\begin{algorithm}[H]
			%\caption{EFF-COMM}
			%\label{effective_approach}
			\label{naive_and_effective_approach}
			\begin{algorithmic}[1]
				\label{algo:NAIVEs-COMM}
				\REQUIRE $M$ layers, graph $G_{\{1, \cdots, M\}}$, $N$ analyses, $K$ related layers on average
				\ENSURE return $L$ - a list of communities
				\STATEx // Algorithm 1a: \textbf{NAIVE-COMM}
				\FORALL {N analyses, each analysis}
				\STATE \quad $G_{AND}$ $\leftarrow$ $\{G_1$ AND  $G_2$ AND $\cdots$ AND $G_K\}$
				\STATE \quad $L$ = InfoM($G_{AND}$)
				\ENDFOR
				\\\hrulefill
			\end{algorithmic}
			\begin{algorithmic}[1]
            \label{algo:EFF-COMM}
				\STATEx // Algorithm 1b: \textbf{EFF-COMM}
				\STATE \quad Store Communities $\{C_1, \cdots, C_M\}$ = $\{\text{InfoM}(G_1), \cdots ,\text{InfoM}(G_M)\}$
                \IF {Communities are self-preserving}
					\FORALL {N analyses, each analysis}
					\STATE \quad $L$ = $\{C_1 \cap \cdots \cap C_K\}$
					\ENDFOR
                \ENDIF
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
	}
    %TODO: rename Figure to Algorithm.
   \begin{figCaption}
   \caption{Algorithms of \textit{NA\"{I}VE-COMM} and \textit{EFF-COMM}}
   \end{figCaption}
    \label{alg:naive_and_effective_approach}
\vspace{-20pt}
\end{figure}

%\begin{figure*}[ht]
%\begin{minipage}[t]{6cm}%6cm <==========================================
%		\vspace{2pt}
%		\begin{algorithm}[H]
%        
%			\caption{NA\"{I}VE-COMM}
%			\label{naive_approach}
%			\begin{algorithmic}[1]
%            \label{algo:NAIVE-COMM}
%				\REQUIRE M layers, graph $G_{\{1, \cdots, M\}}$, $N$ analyses, $\bar{K}$
%				\ENSURE return $L$ - a list of communities
%                %\STATE \quad
%				\FORALL {N analyses, each analysis}
%				\STATE \quad $G_{AND}$ $\leftarrow$ $\{G_1$ AND  $G_2$ AND $\cdots$ AND $G_K\}$
%				\STATE \quad $L$ = InfoM($G_{AND}$)
%				\ENDFOR
%			\end{algorithmic}
%		\end{algorithm}
%	\end{minipage}%
%	\hfil % <===============================================================
%	\begin{minipage}[t]{9.8cm}%6cm <==========================================
%		\vspace{2pt}
%		\begin{algorithm}[H]
%			\caption{EFF-COMM}
%			\label{effective_approach}
%			\begin{algorithmic}[1]
%            \label{algo:EFF-COMM}
%				\REQUIRE M layers, graph $G_{\{1, \cdots, M\}}$, $N$ analyses, $\bar{K}$
%				\ENSURE return $L$ - a list of communities
%				\STATE \quad Store Communities $\{C_1, \cdots, C_M\}$ = $\{\text{InfoM}(G_1), \cdots ,\text{InfoM}(G_M)\}$
%                \IF {Communities are self-preserving}
%					\FORALL {N analyses, each analysis}
%					\STATE \quad $L$ = $\{C_1 \cap \cdots \cap C_K\}$
%					\ENDFOR
%                \ENDIF
%			\end{algorithmic}
%		\end{algorithm}
%	\end{minipage}
%    %TODO: rename Figure to Algorithm.
%    \caption*{Algorithm of two different approaches: NA\"{I}VE-COMM and EFF-COMM}
%\end{figure*}


%\begin{figure*}[ht]
%\begin{minipage}[t]{6cm}%6cm <==========================================
%		\vspace{2pt}
%		\begin{algorithm}[H]
%        
%			\caption{NA\"{I}VE-COMM}
%			\label{naive_approach}
%			\begin{algorithmic}[1]
%            \label{algo:NAIVE-COMM}
%				\REQUIRE M layers having corresponding graph $\{G_1, \cdots, G_M\}$, number of analyses $N$, $K$ is the mean of the number of related layers for each analysis.
%				\ENSURE return $L$ - a list of communities
%                %\STATE \quad
%				\FORALL {N analyses, each analysis}
%				\STATE \quad $G_{AND}$ $\leftarrow$ $\{G_1$ AND  $G_2$ AND $\cdots$ AND $G_K\}$
%				\STATE \quad $L$ = InfoM($G_{AND}$)
%				\ENDFOR
%			\end{algorithmic}
%		\end{algorithm}
%	\end{minipage}%
%	\hfil % <===============================================================
%	\begin{minipage}[t]{9.8cm}%6cm <==========================================
%		\vspace{2pt}
%		\begin{algorithm}[H]
%			\caption{EFF-COMM}
%			\label{effective_approach}
%			\begin{algorithmic}[1]
%            \label{algo:EFF-COMM}
%				\REQUIRE M layers having corresponding graph $\{G_1, \cdots, G_M\}$, number of analysis $N$,  $K$ is the mean of the number of related layers for each analysis.
%				\ENSURE return $L$ - a list of communities
%				\STATE \quad Store Communities $\{C_1, \cdots, C_M\}$ = $\{\text{InfoM}(G_1), \cdots ,\text{InfoM}(G_M)\}$
%                \IF {Communities are self-preserving}
%					\FORALL {N analyses, each analysis}
%					\STATE \quad $L$ = $\{C_1 \cap \cdots \cap C_K\}$
%					\ENDFOR
%                \ENDIF
%			\end{algorithmic}
%		\end{algorithm}
%	\end{minipage}
%    %TODO: rename Figure to Algorithm.
%    \caption*{Algorithm of two different approaches: NA\"{I}VE-COMM and EFF-COMM}
%\end{figure*}




\begin{itemize}[wide]
\item \textit{NA\"{I}VE-COMM (Alg. 1a):}  In this approach, for every analysis it first generates the composed graph, $G_{AND}$, obtained through ($K$-1) 2-layer \textit{AND}-compositions, on average. On this \textit{AND}-composed layer, we apply the Infomap technique (InfoM) \cite{InfoMap2014} to generate the list of communities, $L$. Thus, for $N$ analyses the complexity of this approach will be $O(N*(AND_{i=1}^{K} G_i  + \text{InfoM}(G_{AND}))$, where $K \leq M$. 
\item \textit{EFF-COMM (Alg. 1b):} Its first step is to generate the communities for each of the $M$ layers by applying Infomap. While generating the communities we also obtain the internal clustering coefficient for each node, which are used to determine if the communities are \textit{self-preserving} or not. %For the Facebook multiplex, the self-preserving property was satisfied as the value of this coefficient was one.
%The cost of performing this step will be a part of generating the layer-wise communities.
If the property of \textit{self-preserving} is satisfied, then for each analysis, to generate the list of communities $L$, for the corresponding \textit{AND}-composition $G_{AND}$, communities from \textit{K} layers are intersected based on nodes. Thus, for $N$ analyses the cost of this approach will be, $O (\sum_{i=1}^{M} (\text{InfoM}(G_i)) + N*\cap_{j=l}^{K-l+1} C_{j})$, where $K \leq M$. This approach has been discussed in detail in \cite{ICCS/SantraBC17}.  
\end{itemize}

In terms of storage space, one needs to store $M$ lists of communities for \textit{EFF-COMM}, whereas in \textit{NA\"{I}VE-COMM}, $N*(AND_{i=1}^{K} G_i)$ graphs need to be stored. Considering both space and time, if the number of analyses, $N$, and the average number of layers required for each analysis, $K$, are low then the one-time cost to perform $M$ %number of
Infomap operations in \textit{EFF-COMM} will dominate and make \textit{EFF-COMM} more expensive as compared to \textit{NA\"{I}VE-COMM}. However, with the increasing values of $N$ and $K$, the efficiency of \textit{EFF-COMM} over \textit{NA\"{I}VE-COMM} improves significantly, as the cost to produce the number of \textit{AND}-composed graphs and applying Infomap that traverses through the edges of each of them, begins dominating. In the worst-case for $N$ = $O(2^M)$ and $K$ = $O(M)$, \textit{NA\"{I}VE-COMM} will perform an exponential number of \textit{AND}-compositions and edge traversal-based Infomap operations whereas, \textit{EFF-COMM} will just perform the cost-effective node intersection of layer-wise communities.


\subsection{Performance Results}
\label{subsec:experiments}

%\begin{itemize}
%\item \textit{Overall savings in space:} Instead of storing the AND- composed layers for analysis, we just store the communities of the 11 individual layers. Thus, reducing the overall storage space requirements.
%\item \textit{Analysis Time Reduced:} 

\begin{wrapfigure}{l}{0.5\textwidth}
\vspace{-20pt}
\centering
%\begin{figure}[ht]
%	\renewcommand{\figurename}{Figure}
%	\centering
	\includegraphics[width=0.5\textwidth]{Eff_2}
% 	\vspace{-0.8cm}
	\caption{Overall reduction in analysis time}
	\label{fig:efficiency}
%\end{figure}
\vspace{-20pt}
\end{wrapfigure}


We used a quad-core 8th generation Intel i7 processor Linux machine with 8 GB memory for our analysis. On the Facebook multilayer network with 11 layers ($M$ = 11), based on Table \ref{tab:computationLayers}  we needed 19 \textit{AND}-compositions ($N$ = 19) each having approximately 3 layers on average ($K$ = 3).

\textit{\textbf{EFF-COMM}} needed a \textit{one-time cost} of 50.214 seconds for generating the layer-wise communities using Infomap, followed by intersecting the necessary layer-wise communities to produce the communities of the required \textit{AND}-compositions in a total time of 0.14 seconds. On the other hand, \textit{\textbf{NA\"{I}VE-COMM}} first generated all the required \textit{AND}-composed layers in 65.762 seconds, followed by applying Infomap on each of them to detect the communities in a total time of 12.758 seconds. As shown in Figure \ref{fig:efficiency}, it was observed that even for a small value of $N$ and $K$, \textit{\textbf{EFF-COMM}} reduced the overall analysis time by approximately \textbf{36\%} as compared to \textit{\textbf{NA\"{I}VE-COMM}} \textbf{(78.52 sec v/s 50.354 sec)}. Thus, it proves the utility of this approach when holistically analyzing such multi-feature datasets. 

Note that the above performance numbers is for a specific analytical query and for \textit{AND} compositions. As the number of layers increase in a query, the computation time as well as the number of layer traversals to construct the single graph increases. Also, when \textit{OR} and \textit{NOT} operators are used, the resulting single graphs increase in size (as compared to the \textit{AND} composition),  in which the performance of \textit{EFF-COMM} will be even much better.
%Clearly, if the number of analyses and increases then the efficiency will further improve as the time taken to produce more AND-composed layers and applying a community detection algorithm will overpower the time taken to perform the required node set intersection operations.

%\end{itemize}

%\begin{wrapfigure}{R}{0.3\textwidth}

%In the absence of such an compositional approach, to answer one of the more complex questions like Q4c, we had to first traverse the individual layers and separately generate and store the 5 AND-composed layers, L1 (Age) AND L6 (OPN), L1 (Age) AND L7 (CON), L1 (Age) AND L8 (EXT), L1 (Age) AND L9 (AGR), L1 (Age) AND L10 (NEU). This step itself would have needed additional space and time. After the generation step, the expensive community detection algorithm would have to traverse these 5 new composed layers to generate the communities for us to analyze. Therefore, for answering Q4c by only using the layer wise communities to produce the communities of the 5 required compositions, we saved \% storage space and \% computational time. Such a saving was observed for every analysis that has been performed in this paper. Thus, proving the efficiency of the multilayer network based approach.
